Comparison of Algorithms for Simple Stochastic Games (Full Version)

Simple stochastic games are turn-based 2.5-player zero-sum graph games with a reachability objective. The problem is to compute the winning probability as well as the optimal strategies of both players. In this paper, we compare the three known classes of algorithms -- value iteration, strategy iteration and quadratic programming -- both theoretically and practically. Further, we suggest several improvements for all algorithms, including the first approach based on quadratic programming that avoids transforming the stochastic game to a stopping one. Our extensive experiments show that these improvements can lead to significant speed-ups. We implemented all algorithms in PRISM-games 3.0, thereby providing the first implementation of quadratic programming for solving simple stochastic games.

==> 3_1_VI.tex <==
This section recalls the results and algorithms of~\cite{KKKW18}, as the extension of quadratic programming uses some similar ideas, and since this paper is about comparing all types of algorithms.

\todo{find a better place for the "why we compute upper bound"; not in the middle of some paragraph. Better: First VI vs. BVI, then describe.}
\todo{what about topological BVI? $->$ introduce as contribution. Restructure: First describe all, then opts: Warm start for SI and QP, topological for SI and VI, other stuff for QP}
The basic idea of bounded value iteration (BVI) is to start from a vector $\lb<0>$/$\ub<0>$ that is definitely an under-/over-approximation of the value, i.e. for every state $\lb<0>(\state) \leq \val(\state) \leq \ub<0>(\state)$.
Then the algorithm repeatedly applies so called \emph{Bellman updates}, i.e. it uses a version of Equation \ref{eq:Vs} as follows (the equation for the over-approximation is obtained by replacing $\lb$ with $\ub$):
\begin{equation}\label{eq:Ls}
\lb<n>(\state) =  \begin{cases} 
\max_{\action \in \Av(\state)}\lb<n-1>(\state,\action)		&\mbox{if } \state \in \states<\Box>  \\
\min_{\action \in \Av(\state)}\lb<n-1>(\state,\action) &\mbox{if } \state \in \states<\circ>
\end{cases},
\end{equation}
where $\lb<n-1>(\state,\action)$ is computed from $\lb<n-1>(\state)$ as in Equation \ref{eq:Vsa}.
Since $\val$ is the least fixpoint of the Bellman equations, $\lim_{n \to \infty} \lb<n>$ converges to $\val$.
However, to be certain that $\lb$ has converged, we need to perform an exponential number of iterations~\cite{visurvey}.
Computing an over-approximation is quicker, but it need not converge to $\val$, because it might stay at some greater fixpoint of the Bellman equations.

\begin{example}\label{ex:ubNoConvergeVI}
	Consider the SG of Figure \ref{fig:SGex} with the EC $\{\mathsf p, \mathsf q\}$. Let $\ub<0> = 1$ for $\mathsf p$, $\mathsf q$ and $\target$ and $\ub<0> = 0$ for $\sink$.
	Then we have $\ub<0>(\mathsf q, \mathsf b) = 1$ and $\ub<0>(\mathsf q, \mathsf c) = \sfrac 2 3$. Thus, $\mathsf q$ will pick action $\mathsf b$, as it promises a higher value, and the over-approximation does not change.
	This happens, because looking at the current upper bound, Maximizer is under the impression that staying in the EC yields a higher value. However, it actually reduces the probability to reach the target to 0.
	So the algorithm has to perform an additional step to inform states in an EC that they should not depend on each other, but on the best exit.
	In this case, $\ub<1>(\mathsf q) \eqdef \bE<\ub<0>>[\Box](\{\mathsf p,\mathsf q\}) = \ub<0>(\mathsf q, \mathsf c) = \sfrac 2 3$.
\end{example}

In fact, it does not suffice to only decrease the upper bound of ECs, but a more in depth graph analysis is required to detect the real problem, so called \emph{simple end components} (SEC)~\cite{KKKW18}.
Decreasing the value of those SECs to their best exit repeatedly results in a convergent over-approximation. 
We recall the full algorithm in Algorithm \ref{alg:bvi}.\todo{align comments}

\begin{algorithm}[htbp]
	
	\caption{Bounded value iteration algorithm from \cite{KKKW18}}\label{alg:bvi}
	\begin{algorithmic}[1]
		\Procedure{BVI}{precision $\epsilon>0$}
		\For {$\state \in \states$} \Comment{Initialization}
		\State $\lb(\state)=0$ ~~\Comment{Lower bound}
		\State $\ub(\state)=1$ ~~\Comment{Upper bound}
		\EndFor
		\State \textbf{for} $\state \in \fstates$ \textbf{do} $\lb(\state) = 1$ \Comment{Value of targets is determined a priori}
		
		\medskip
		
		\Repeat
		\State $\lb,\ub$ get updated according to Eq.~(\ref{eq:Ls}) \Comment{Bellman updates}
		\smallskip
		\For{$T \in \FIND$} \Comment{For every SEC}
			\For {$\state \in T$} 
				\State $\displaystyle \ub(\state) \gets  \bE<\ub>[\Box](T)$\label{line:adjust} \Comment{Decrease upper bound to best exit}
			\EndFor
		\EndFor
		\Until{$\ub(\initstate) - \lb(\initstate) < \epsilon$}
		\Comment{Guaranteed error bound}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

Term crit: Right now only written for $\initstate$, but we could also iterate until all states have converged. Then we can also infer the $\varepsilon$-optimal strategy.

There also is a simulation based asynchronous version of BVI which can perform very well on models where only a small part of the state space is relevant for convergence. 
It is based on \cite{atva} and described in \cite[Section 4.4]{KKKW18}. We also experimentally compare to it, but refrain from explaining it here as that is not the point of the paper.\todo{improve this, as well as the first paragraph where I say why we describe VI. Also intro should motivate this.}

==> 3_2_QP.tex <==
\todo{restructure a lot} 
4.1 Lifting the constraints of CNF
Show Condon QP. State assumptions of CNF one by one, what they are used for and how we can replace them. Then have another paragraph for each assumption.
In the end, since we lifted the assumptions, we reduced the size of the input to the QP, and hence made it practical.
Size of QP can be exp, because of MEC business. Solving QP takes exp time currently, too.
However, easily can give nondet poly algo.

4.2 Improvements
Warm start.
If SI comes first, I can just refer to the opt section here.

Using \emph{quadratic optimization} for solving simple stochastic games was introduced by Condon \cite{DBLP:conf/dimacs/Condon90}. The proposed \emph{quadratic program (QP)} requires the $\SG$ to be in a certain normal form, which we refer to as \emph{\cnf{}}. The necessary procedures to transform an arbitrary $\SG$ into one in \cnf{} were given in \cite{condonComplexity}, and we recall them in Appendix \ref{app:cnf}

%Although this approach usually is regarded as inefficient, there has been no implementation of Condon's approach prior to this paper. We provide an implementation of \conQP{}, and we improve it by eliminating unnecessary transformations and by adjusting the QP. Furthermore, we compare our improved QP to Strategy Iteration, Bounded Value Iteration, and Value Iteration.

The proofs to the lemmata and theorems are provided in the appendix \ref{qpProofs}.

\subsection{Condon's quadratic program}
We review \conQP{} briefly and discuss then how we can discard or improve them.

A $\SG$ satisfies \cnf{} if it has following form:
\begin{enumerate}
		\item ($\twoSucc$) For all $\state \in \states : |\Av(\state)| \leq 2$,
		\item ($\halfProbs$) For all $\state \in \states , \action \in \Av(\state), \state' \in \states: \trans(\state,\action,\state') \in \{0, 0.5, 1\}$, 
		\item ($\stopping$) Given $\SG$ must be a stopping game
		\item ($\noOneSucc$) if $|\Av(\state)| = 1$ then $\state$ is a target or a sink
\end{enumerate}

Each of the requirements comes with an own transformation that is provided in the appendix \ref{transforms}

The quadratic program solving an $\SG$ in \cnf{} is:
\begin{equation*}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_
{\substack{\state \in \states \\ \Av(\state) = \{\action, \actionb\}}}
(\val(\state) - \val(\state,\action)) (\val(\state) - \val(\state,\actionb))&&\\
\text{subject to}& 
\displaystyle\val(\state) \geq \ \val(\state,\action) &\forall \state \in \states<\Box>: |\Av(\state)| = 2, \forall \action \in \Av(\state) &\\
& \displaystyle\val(\state) \leq \ \val(\state,\action)  &\forall \state \in \states<\circ>: |\Av(\state)| = 2, \forall \action \in \Av(\state) &\\
& \displaystyle\val(\state) = 1  &\forall \state \in \fstates &\\
& \displaystyle\val(\state) = 0  &\forall \state \in \sink &\\
& \displaystyle\val(\state) \in [0,1] \subset \mathbb{Q}  &\forall \state \in \states &\\ 
\end{array}
\end{equation*}
\begin{equation*}
\text{where}\; \; \val(\state,\action) = \left\{\begin{array}{ll}
        \val(\mathsf{s} ') & \text{for } |\post(\state, \action)| = \{\mathsf{s} ' \}\\
        \frac{1}{2} \val(\mathsf{s} ') + \frac{1}{2} \val(\mathsf{s} '') & \text{for } |\post(\state, \action)| = \{\mathsf{s} ', \mathsf{s} '' \}
        \end{array}\right\}
\end{equation*}
Note that this is not the exact quadratic program that Condon has written down in \cite{DBLP:conf/dimacs/Condon90}, but we reformulated it so that it fits our notations and definitions.
To reach the only local minimum in the constraint region the objective value has to be 0. In this case the strategies $\straa, \strab$ are optimal~\cite{DBLP:conf/dimacs/Condon90}.



\subsection{Improvements}
Every transformation adds additional states or actions to the $\SG$ and increases the time necessary to solve the QP considerably. We simplify the QP to accept more arbitrary $\SG$s as input. We do so by going from Condon's constraint-matrix to one that accepts more general $\SG$s and by proving that every step is correct.

\subsubsection{2Act}
The only requirement we do not change is that every state may have atmost two actions. We do so to keep the objective function quadratic. If we allow for more than two actions, the objective function has to be rewritten to handle states with an arbitrary amount of actions correctly. This gives rise to a polynomial optimization problem, which can be solved with \textcolor{red}{RAPOSA, BARON, (AMPL is just a language that uses then Baron/Raposa, not a solver itself)}.

\subsubsection{No1Act}
The $\noOneSucc$-constraint compels every state $\state \in \states$ that is not absorbing to have only one action. To this end, we search for every state $\state$ that is not absorbing and has exactly one action and add a second action leading to either a sink or a target depending on whether $\state \in \states<\Box>$ or $\state \in \states<\circ>$. Every additional action makes the quadratic program more difficult to solve since every action is represented as one constraint, and every state with two actions expands the objective function. For this reason, it is beneficial to drop the $\noOneSucc$-constraint.

\begin{lemma}[dropNo1Act]\label{dropNo1Act}
Let $\state \in \states$ be a state in a $\SG$ with two actions $\action$ and $\actionb$: $\action$ is the action $\state$ originally had, and $\actionb$ is the additional action inserted to comply with $\noOneSucc$.

Then it holds that $\val(\state) = \val(\state,\action)$.
\end{lemma}

We conclude that every state $\state \in \states$ with only one action does not require a second action that never optimizes the value of $\state$. Thus, we can drop the $\noOneSucc$-constraint. Instead, we can add the following constraint to the QP:
\[
	\forall \state \in \states: \Av(\state) = \{\action \}: 
	\val(\state) = \val(\state,\action)
\]

\subsubsection{Half-probabilities}
To comply with the $\halfProbs$-requirement, every transition $\trans(\state, \action, \state')$ with $\state, \state' \in \states$ and $\action \in \Av(\state)$ must have a probability of 0, 0.5 or 1. 

For the transformation of a $\SG$ into one that complies with $\halfProbs$, we pick state-action pairs ($\state, \action$) with $\state \in \states , \action \in \Av(\state)$ that do not have fitting transition probabilities and construct a corresponding binary tree. Every inner node of the binary tree has only one action with the required transition probabilities. Since we have seen in Lemma \ref{dropNo1Act} that it is not necessary to provide a second action for the inner nodes, we assume they have just one.

We explain now, why we do not require the $\SG$ to comply with $\halfProbs$ and that we can use arbitrary rational transition probabilities instead so that $\val(\state,\action) = \valSum$.

Let $v \in \states$ be a state with only one action $\action$. The value of $v$ is $\val(\state) = \sum\limits_{v_i \in \post(v,\action)} \trans(v, \action\, v_i) \cdot \val(v_i)$. If $v \neq \initstate$ we redirect all actions from other states $\state \neq v$ leading to $v$ directly to the successors of $v$.

\begin{lemma}[dropHalfProbs] \label{dropHalfProbs}
Let $\state$ be a state in a $\SG$ $\SGinstance$ with an action $\action$. ($\state, \action$) has a transition leading to state $v$ with transition probability $\delta_{v}$, where $\state \neq v \neq \initstate$. Let $v$ have \emph{exactly one} action $\action$ that has probability 0 of leading back to v: $v \notin \post(v, \action)$.

Then there exists a $\SG$ 
$\SGinstance ' = (\states \setminus \{v\},\states<\Box> \setminus \{v\},\states<\circ> \setminus \{v\},\initstate,\actions,\Av,\delta ')$ with a transition probability function $\delta '$, where $\delta '(\state<i> ,\action ,\state ') = \trans(\state<i> ,\action ,\state ' ) + \delta(\state<i> ,\action ,v) \cdot \trans(v ,\action ,\state ' )$ for all $\state<i> \in \states \setminus \{v\}$, $\action \in \Av(\state<i>)$, $\state ' \in \post(\state<i> ,\action)$.

Note that for every state-action pair ($w, \actionb $)$ \neq $($\state, \action $) every transition probability is equal to $\delta$ because $\delta(w ,\actionb ,v) = 0$. Furthermore, it holds that $\val<\SGinstance>(\state<i>) = \val<\SGinstance'>(\state<i>)$ for every state $\state<i> \in \states \setminus \{v\}$.
\end{lemma}

Due to this lemma, we can reverse the $\halfProbs$-transformation into the original $\SG$ by iteratively removing the inner nodes of the trees, as they only have one action with a transition probability of 0 of leading to themselves. We preserve the value of every state of the original $\SG$. Now we need to rephrase the QP to allow arbitrary rational transition probabilities.

We drop the $\halfProbs$-constraint and rewrite in \conQP{} $\val(\state, \action)$ as $\valSum$ for stopping $\SG$s that comply with $\twoSucc$ as. The resulting QP is:
\begin{equation*} \label{eq:ourQP}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_
{\substack{\state \in \states \\ \Av(\state) = \{\action, \actionb\}}} 
(\val(\state) - \val(\state, \action))\cdot
(\val(\state) - \val(\state, \actionb))&\\
\text{subject to}& 
\displaystyle\val(\state) \geq \ \val(\state,\action) &\forall \state \in \states<\Box>: 
|\Av(\state)| = 2, \forall \action \in \Av(\state) &\\
& \displaystyle\val(\state) \leq \ \val(\state,\action) &\forall \state \in \states<\circ>: 
|\Av(\state)| = 2, \forall \action \in \Av(\state) &\\
& \displaystyle\val(\state) = \ \val(\state,\action)  &\forall \state \in \states: \Av(\state) = \{\action \}&\\
& \displaystyle\val(\mathsf{f}) = 1  &\forall \mathsf{f} \in \fstates &\\
& \displaystyle\val(\mathsf{\state}) = 0  &\forall \mathsf{\state} \in \sink &\\
& \displaystyle\val(\state) \in [0,1] \subset \mathbb{Q}  &\forall \state \in \states &\\ 
\text{where} & \displaystyle\val(\state,\action) = \valSum & 
\forall \state \in \states, \forall \action \in \Av(\state) &\\
\end{array}
\end{equation*}
The mathematical program has only linear constraints and only quadratic objective terms. Thus, we still have a quadratic program with linear constraints.

\begin{theorem}[correctnessQP] \label{correctnessQP}
Let $\SGinstance$ be an arbitrary stopping $\SG$ that complies with the $\twoSucc$-constraint.

The quadratic program with linear constraints (\ref{eq:ourQP}) computes the optimal value of every $\state \in \states$ in $\SGinstance$.
\end{theorem}

With this theorem, we have provided a QP that requires fewer constraints than \conQP{} and therefore reduces the blowup of states and actions drastically.

\subsection{Handling end components}
The last constraint of \cnf{} is that we require the $\SG$ to be stopping. For the transformation of arbitrary games into stopping games, one must insert in every transition a small probability $\epsilon < 1/4^{|\states| -1}$ that this transition leads directly to a sink \cite{shapley}\cite{condonComplexity}. To add the $\epsilon$-transitions and still comply with the rest of \cnf{}, $\epsilon$ is represented by a chain of $m$ new states per action. $m$ must be sufficiently large to have no impact on the value of the $\SG$. Since $\epsilon < 1/4^{|\states| -1}$ it holds that $m > 2(|\states |-1)$ due to $\epsilon = 1/2^{m}$. Since this approach is specifically designed to handle end components, it is reasonable to insert the $\epsilon$-transitions only into actions of states that are in MECs. This way, we manipulate the value of the game lesser and ensure that every MEC will still be left almost surely. \textcolor{red}{Not sure whether the following 2 sentences are correct/relevant} Furthermore, we can allow probably for an even bigger $\epsilon$ since we could reduce the MEC to a subgame on its own and the corresponding $\states '$ would be smaller. However, since a smaller $\epsilon$ has less influence on the value of the game, we decide to keep $\epsilon < 1/4^{|\states| -1}$.

While this concept is correct in theory, it is not a viable approach to handle end components. The introduced $\epsilon$ is so small that the quadratic optimizers we use are not capable of handling it correctly and produce incorrect results.

\begin{example}
\input{examplesQP/BigMec}
We consider as an example the model "BigMec" with $N = 3$, which is a model with one target, one sink, and one scalable MEC. Figure \ref{ex:bigMec} illustrates "BigMec" with $N=2$. There are $2N$ Maximizer states in the MEC. According to Condon it must hold that $\epsilon < 1/4^{9 -1}$. We compute $\val(\initstate)$ for $\epsilon = 1/2^{17}$ in Gurobi Optimizer 9.0 \cite{gurobi} \textcolor{red}{THIS HAS NO DOI, NOT SURE IF TO INSERT AS CITE} with every tolerance parameter set to highest precision.
The computed value is 0.49935%34020591185
\ instead of the 0.4 it truly should have. While it is natural to assume that the $\epsilon$ was chosen too big, smaller epsilons yield even less accurate solutions.
\end{example}

Thus, we take another approach of setting up additional constraints for MECs so that the resulting quadratic program solves both stopping and non-stopping games correctly. We can distinguish between the cases where the MEC contains only $\circ$-vertices, only $\Box$-vertices or both.

In every MEC that only contains $\circ$-vertices, the value of every state is 0, since there is a strategy that never leaves the MEC and therefore no target is reached. To capture this, we introduce following constraint to the QP:
\[
\val(\state) = 0  \quad \forall \state \in T \in \mec(\G): T \cap \states<\Box> = \emptyset
\]

Whenever a MEC contains only $\Box$-vertices, every state can go for the bestExit. To compute the bestExit of a MEC $T$ with only $\Box$-vertices in a simple stochastic game $\SGinstance$, we iterate over every $\state \in T$ and every action $\action \in \Av(\state)$ that leaves $T$ and assign to the value each of state $\state '$ in $T$ the maximum of each $\val(\state,\action)$. Thus, we add the constraint
\begin{equation} \label{eq:bestExitFirstApproach}
\begin{aligned}
\forall \state, \state' \in T & \in \mec(\SGinstance): T \cap \states<\circ> \cap \fstates = \emptyset:\\ 
	&\val(\state') = \max_{(\state, \action) \leaves T} \val(\state, \action) \\
\end{aligned}
\end{equation}
to the QP. This ensures that every state $\state \in T$ has the value of the bestExit. Note that max- and min-constraints are expressed through continous and boolean variables. Therefore, the resulting quadratic program is a mixed-integer program.

\subsubsection{MECs containing vertices of both players}
Should the MEC contain vertices of both players, neither of the approaches above yields the sufficient constraints.

The inherent problem with MECs is that the values of their states are mutually dependent on each other. For example in Figure \ref{SGex}, as long as $p$ and $q$ the same value, they may choose any value $\frac{1}{3} \leq v \leq 1$ and \conQP{} would consider it optimal, although their value is obviously $\frac{1}{3}$. This problem occurs neither in states that are in no MECs nor in absorbing states. Futhermore, we know that MECs that contain states of both players never include absorbing states. Thus, we can  express the value $\val(\state)$ for every state $\state$ in a MEC $T$ depending on its exits $\exits$ and thereby avoid the problem.
%\input{examples/exampleMC}

%Figure \ref{ex:exampleMC} illustrates an example where states $\{m_0, m_1, m_2\}$ are a MEC. States $\{s_3, s_4\}$ are exits of the MEC. The value of the states $\{m_0, m_1, m_2\}$ in $\G[\straa,\strab]$ can be described depending only on the exits. For example $\valstra (m_0) = p_{m_0}^{\straa ,\strab} (s_3) \cdot \valstra (s_3) + p_{m_0}^{\straa,\strab} (s_4) \cdot \valstra (s_4)$.

To this end we iterate over every possible strategy-pair ($\straa, \strab$), induce the corresponding Markov chain $\G[\straa ,\strab]$ and express $\valstra (\state)$, $\state \in T$ depending on the exits $\exits$ of $T$. Then we add the constraints $\val(\state) = \max\limits_{\straa}\min\limits_{\strab}\valstra(s)$ to the QP.

Since in every induced Markov chain $\G[\straa ,\strab]$ we are only interested in states $\state \in T$ we can consider just the Markov chain $\G<\Tinstance>[\straaT ,\strabT]$ induced by fixing strategies on a smaller simple stochastic game $\Tinstance = (T \cup \exits, T_{\Box} \cup \exits_{\Box}, T_{\circ} \cup \exits_{\circ},m_0,\actions,\Av',\delta ')$ with $m_0 \in T$. As we do not care what happens after reaching an exit $e \in \exits$ for expressing $\valstra (\state)$, we model the exits as targets. Therefore every exit has only one action, which is a self-loop with transition probability one.
For every state $\state \in T$ it holds that $\Av(\state) = \Av'(\state)$ and $\trans(\state, \action, \state') = \trans'(\state, \action, \state')$ for every $\action \in \Av'(\state)$ and $\state' \in T \cup \exits$. This way we don't need to iterate over every strategy-pair ($\straa, \strab$) but only the strategies ($\straaT, \strabT$) of every state $\state \in T$.

To ensure that we do not need to the rest of the original $\SG$ to compute the values for a fixed strategy-pair in $\G<\Tinstance>[\straaT ,\strabT]$, we consider following lemma:

\begin{lemma}[exitDependency] \label{exitDependency}
Let $T$ be a MEC in $\SG$ with at least one state of each player and let $\exits$ be the set of exit-states out of $T$. Let $\straaT ,\strabT$ be strategies that are only defined for $\state \in T$. Let furthermore $\straaST , \strabST$ be the strategies defined for every state $\state ' \in \states$ that use $\straaT ,\strabT$ for $\state \in T$. Then for each $\state \in T$ it holds that for fixed strategies $\straaT ,\strabT$ the value of $\state$ is
\[
	\val<\straaT ,\strabT>(\state) = \sum\limits_{e \in \exits}p_s^{\straaT ,\strabT}(e) \cdot \val<\straaT ,\strabT>(e)
\]
Where $\val<\straaT ,\strabT>(e)$ is the optimal value of $e \in \exits$ for fixed strategies $\straaT, \strabT$, i.e. $\val<\straaT, \strabT>(e) = \max\limits_{\straaST}\min\limits_{\strabST}\val<\straaST, \strabST>(e)$ where states $\state \in T$ use $\straaT, \strabT$.
\end{lemma}

We want the probabilities $p_{\state}^{\straa, \strab}(e)$ of state $\state \in T$ reaching the absorbing exits $e \in \exits$ in $\G<\Tinstance>[\straaT, \strabT]$. We can compute $p_{\state}^{\straaT, \strabT}(e)$ with all-pairs shortest path algorithms like the Flyod-Warshall algorithm.

\begin{theorem}[orderInvariance] \label{orderInvariance}
Let state $\state$ be in MEC $T$ in a $\SG$, where $T$ has at least one state of both players. Then
\[
	\val(\state) = \max\limits_{\straaT}\min\limits_{\strabT}\val<\straaT, \strabT>(\state)
\]
\end{theorem}

Therefore, we can add following constraint to our QP for every MEC $T$ that has at least one state of each player and for every strategy-pair ($\straaT, \strabT$) in $T$:
\[
	\forall \state \in T: \val<\straaT, \strabT>(\state) = \sum\limits_{e \in \exits}p_s^{\straaT, \strabT}(e) \cdot \val<\straaT, \strabT>(e)
\]

As MECs tend to appear rarely and in small size in models, this is a significant improvement to iterating over every possible strategy-pair. However, note that in the worst case we have to consider $2^{|\states \setminus (\fstates \cup \sink)|}$ strategy-pairs.

\subsection{NP-Completeness}
\todo{Just say: Runtime is exp (e.g. if everything is a MEC; we try all strategies...). With slight changes, it runs in nondeterministic polynomial time, as we can guess the strategy in the MEC, the QP is of polynomial size and solving QP is in NP.}
Since solving a quadratic program is known to be $\nptime$-complete \cite{qpNPcomplete}, we only need to prove that building the QP from the $\SG$ is done in $\nptime$. Following steps can be done in polynomial time by a deterministic Turing-machine:
\begin{itemize}
	\item Preprocessing the $\SG$ by computing the attractors of the targets and the sinks since it's a backwards depth-first search from the targets and the sinks,
	\item Applying the 2Act-transformation \cite{condonComplexity} and
	\item Computing $\mec(\G)$
\end{itemize}  

Setting up the constraints for each state that is not in a MEC can be done in $O(|\states |^2)$ since every state may have at most two actions that have a transition to every state. The objective function is takes also constructed in $O(|\states |^2)$ as every value $\val(\state, \action)$ for $\action \in \Av(\state)$ is subtracted from $\val(\state)$, and $\val(\state, \action)$ is depending on at most $|\states | -1$ states.

Let $T$ be a non-deterministic Turing machine. Since we can use $M$ to guess the optimal strategy-pair ($\straa, \strab$) we do not have to iterate over all the exponentially many strategy-pairs. We can then set $\val(\state)$ to $\valstra (\state)$. \textcolor{red}{BUT WHAT ABOUT THE POLYNOMIAL CERTIFICATE?}

Thus we know that building the corresponding QP from a $\SG$ is in $\nptime$ and, the that whole algorithm to solve a $\SG$ with our improved approach is $\nptime$-complete.


%\subsubsection{Setting up the correct constraints for one strategy-pair}

%Until now, we have always constructed the Markov chain $\G[\straa,\strab]$ for the whole $\SG$. However, since we are only interested in expressing $\valstra (\state), \state \in T$ depending on the exits $\exits$, we may consider just the Markov chain $\G<\Tinstance>[\straaT ,\strabT]$ induced by fixing strategies on a smaller simple stochastic game $\Tinstance = (T \cup \exits, T_{\Box} \cup \exits_{\Box}, T_{\circ} \cup \exits_{\circ},m_0,\actions,\Av',\delta ')$ with $m_0 \in T$. As we do not care what happens after reaching an exit $e \in \exits$, we model the exits as targets. Therefore every exit has only one action, which is a self-loop with transition probability one. 
%For every state $\state \in T$ it holds that $\Av(\state) = \Av'(\state)$ and $\trans(\state, \action, \state') = \trans'(\state, \action, \state')$ for every $\action \in \Av'(\state)$ and $\state' \in T \cup \exits$.

%\subsubsection{Setting up the correct constraints all strategy-pairs}
%We handle MECs that have strategy fixed correctly. Now we need to iterate over every strategy-pair we can assign to the states in the MEC and set up the constraints for $\val(\state)$ for each $\state \in T$ depending on the exits $e \in \exits$. We need to ensure first that if we iterate over every strategy-pair in the MEC, we get the optimal value of $\state \in \states$.

%\begin{theorem}
%Let state $\state$ be in MEC $T$ in a $\SG$, where $T$ has at least one state of both players. Then
%\[
%	\val(\state) = \max\limits_{\straaT}\min\limits_{\strabT}\val<\straaT,
%\strabT>(\state)
%\]
%\end{theorem}
%We can add following constraint to the QP for all MECs $T$ in the $\SG$ with at least one state of each player:
%\[
%	\forall \state \in T: \val(\state) = \max\limits_{\straaT}\min\limits_{\strab _T}\val<\straa _T, \strabT>(\state)
%\]
%We describe every value $\val(\state)$ of a state $\state \in T$ depending on the exits and can compute the values correctly. Note that the number of constraints increases exponentially in the number of actions in the MEC. Therefore, our approach to solving non-stopping games is not in $\nptime$, but in $\exptime$ if $\nptime \subsetneq \exptime$. However, we do not need $2^{|\states|}$ iterations, but only $\sum\limits_{T: MEC \in \SGinstance}2^{|T|}$ if $\SGinstance$ is a $\SG$ and every state $\state \in T$ has two actions.

\subsection{Further optimizations}
\subsubsection{QP warm starts}
To improve the runtime of Gurobi Optimizer on the examples that require hours or days to be solved, we provide an initial solution (also called \emph{warm start}) that it is close to the optimum. We can obtain such an initial solution by using unbounded value iteration.

However, there are several problems why this does not yield faster solutions: On one hand, the solution provided by unbounded value iteration may be infeasible for the QP and be discarded. On the other hand, Gurobi Optimizer provides its ways to find initial solutions that tend to perform as well as it would with the precomputed warm start from unbounded value iteration.

In none of the experiments did the QP with warm starts from unbounded value iteration perform significantly better than the QP without the warm start.
\todo{find good place for this opt}

%TODO: Sasha: Try to condense the information from your thesis into 3 pages. Proofs can be delegated to appendix. Try to convey the ideas we had, why they are good and how they work; state the lemmata/theorems for correctness, but don't put the proofs.

%Also put all the other stuff that you have (currently in the text file) here.

%Use subsections as you see fit, but don't invest too much into that. 
%We will probably restructure anyway.

==> 3_main.tex <==
\section{Algos state of the art}

\subsection{VI}

\subsection{SI}

How to solve MDP (approx) [where to put?] cite(KM17)

\subsection{QP}
App: How to transform. 

\section{Optimizations}

\subsection{CNF replacement}
Dropping all constraints one by one.
cite(condon)

\subsection{Warm start}
cite(KM17)

\subsection{Topological}
cite(KM17, topological, ensuring)


%\section{Value iteration}\label{sec:VI}
\input{3_1_VI}

%\section{Strategy Iteration}\label{sec:SI}
\input{3_3_SI}

%\section{Quadratic Programming}
\input{3_2_QP}






